Orderly Management of Packets in RDMA by Eunomia

To fulfill the low latency requirements of today's applications, deployment of RDMA in datacenters has become prevalent over the recent years. However, the in-order delivery requirement of RDMAs prevents them from leveraging powerful techniques that help improve the performance of datacenters, ranging from fine-grained load balancers to throughput-optimal expander topologies. We demonstrate experimentally that these techniques significantly deteriorate the performance in an RDMA network because they induce packet reordering. Furthermore, lifting the in-order delivery constraint enhances the flexibility of RDMA networks and enables them to employ these performance-enhancing techniques. To realize this, we propose an ordering layer, Eunomia, to equip RDMA NICs to handle packet reordering. Eunomia employs a hybrid-dynamic bitmap structure that efficiently uses the limited on-chip memory with the help of a customized memory controller and handles high degrees of packet reordering. We evaluate the feasibility of Eunomia through an FPGA-based implementation and its performance through large-scale simulations. We show that Eunomia enables a wide range of applications in RDMA datacenter networks, such as fine-grained load balancers which improve performance by reducing average flow completion times by 85% and 52% compared to ECMP and Conweave, respectively, or employment of RDMA in expander topologies like Jellyfish which allows up to 60% lower flow completion times and higher throughput gains compared to Fat tree.

==> Future_Work/future_work.tex <==
\textbf{PFC Aware Load Balancer: } We observed in \S \ref{eval_fine_grain_lb} that DRILLs performance is affected due to PFC because DRILL tracks the last best path that a packet is sent to, and routes more packets on that path if it remains locally best among the two randomly picked paths. However, a seemingly good local decision can lead to a PFC paused path. This leads to longer delays due to PFC, which can be observed in Fig \ref{fig:pfc_clos_ali}. It would be worthwhile to explore load balancing that takes into account the PFC triggers and avoids sending packets on paths that are facing PFC pause to reduce the impact of PFC on performance. With Eunomia, the load balancing does not have to be limited by coarse granularity.

\textbf{Practical Implementation: } The next step for this project would be to implement Eunomia on programmable switches, and evaluate 
